Trees from Functions as Processes

Levy-Longo Trees and Bohm Trees are the best known tree structures on the {\lambda}-calculus. We give general conditions under which an encoding of the {\lambda}-calculus into the {\pi}-calculus is sound and complete with respect to such trees. We apply these conditions to various encodings of the call-by-name {\lambda}-calculus, showing how the two kinds of tree can be obtained by varying the behavioural equivalence adopted in the {\pi}-calculus and/or the encoding.

==> shortBIB.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }

\bibitem{A-KHe92}
Arun-Kumar, S., Hennessy, M.: An efficiency preorder for processes. Acta
  {I}nformatica  29,  737--760 (1992)

\bibitem{Bar84}
Barendregt, H.P.: The Lambda Calculus:  Syntax, semantics. North-Holland
  (1984)

\bibitem{BergerHY01}
Berger, M., Honda, K., Yoshida, N.: Sequentiality and the pi-calculus. In:
  Proc. TLCA'01. LNCS, vol. 2044, pp. 29--45. Springer (2001)

\bibitem{BergerHY05}
Berger, M., Honda, K., Yoshida, N.: Genericity and the pi-calculus. Acta {I}nformatica 
  42(2-3),  83--141 (2005)

\bibitem{DemangeonH11}
Demangeon, R., Honda, K.: Full abstraction in a subtyped pi-calculus with
  linear types. In: Proc. CONCUR'11. LNCS, vol. 6901, pp. 280--296.  Springer (2011)

\bibitem{DezG01}
Dezani-Ciancaglini, M., Giovannetti, E.: From Bohm's theorem to observational
  equivalences: an informal account. ENTCS.  50(2),
  83--116 (2001)

\bibitem{HMS12}
Hirschkoff, D., Madiot, J.M., Sangiorgi, D.: Duality and i/o-types in the
  $\pi$-calculus. In: Proc.\ CONCUR'12. LNCS, vol. 7454, pp. 302--316. Springer
  (2012)

\bibitem{Mil89}
Milner, R: Communication and Concurrency. Prentice Hall, 1989.

\bibitem{Mil92}
Milner, R.: Functions as processes. Mathematical Structures in Computer Science
   2(2),  119--141 (1992) %, research Report 1154, INRIA, Sofia Antipolis, 1990

\bibitem{Mil99}
Milner, R.: Communicating and Mobile Systems: the $\pi$-Calculus. CUP (1999)

\bibitem{Plo78}
Plotkin, G.D.: ${T}^\omega$ as a universal domain. Journal of Computer and
  System Sciences  17,  209--236 (1978)

\bibitem{San95lazy}
Sangiorgi, D.: Lazy functions and mobile processes. In: Proof, Language and Interaction: Essays in Honour of
  Robin Milner.  pp. 691--720. {MIT} {P}ress (2000)

\bibitem{SW01a}
Sangiorgi, D., Walker, D.: The $\pi$-calculus: a Theory of Mobile Processes.
CUP (2001)

\bibitem{Sco76}
Scott, D.: Data types as lattices. SIAM Journal on Computing  5(3),  522--587
  (1976)

\bibitem{YoshidaHB07}
Yoshida, N., Honda, K., Berger, M.: Linearity and bisimulation. Journal of Logic and Algebraic Programming  72(2),  207--238 (2007)

\end{thebibliography}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

